Sequential infinite-dimensional Bayesian optimal experimental design with derivative-informed latent attention neural operator

We develop a new computational framework to solve sequential Bayesian optimal experimental design (SBOED) problems constrained by large-scale partial differential equations with infinite-dimensional random parameters. We propose an adaptive terminal formulation of the optimality criteria for SBOED to achieve adaptive global optimality. We also establish an equivalent optimization formulation to achieve computational simplicity enabled by Laplace and low-rank approximations of the posterior. To accelerate the solution of the SBOED problem, we develop a derivative-informed latent attention neural operator (LANO), a new neural network surrogate model that leverages (1) derivative-informed dimension reduction for latent encoding, (2) an attention mechanism to capture the dynamics in the latent space, (3) an efficient training in the latent space augmented by projected Jacobian, which collectively leads to an efficient, accurate, and scalable surrogate in computing not only the parameter-to-observable (PtO) maps but also their Jacobians. We further develop the formulation for the computation of the MAP points, the eigenpairs, and the sampling from posterior by LANO in the reduced spaces and use these computations to solve the SBOED problem. We demonstrate the superior accuracy of LANO compared to two other neural architectures and the high accuracy of LANO compared to the finite element method (FEM) for the computation of MAP points and eigenvalues in solving the SBOED problem with application to the experimental design of the time to take MRI images in monitoring tumor growth. We show that the proposed computational framework achieves an amortized $180\times$ speedup.

==> ex_shared.tex <==

% Packages and macros go here
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{braket}
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\usepackage{multirow}
\usepackage{subcaption}
\usepackage{amsopn}
\usepackage{algorithm}
\usepackage{color}
\usepackage{hyperref}

\DeclareMathOperator{\diag}{diag}

\newcommand{\bE}{{\mathbb{E}}}
\newcommand{\bI}{{\mathbb{I}}}
\newcommand{\bN}{{\mathbb{N}}}
\newcommand{\bR}{{\mathbb{R}}}

\newcommand{\cA}{{\mathcal{A}}}
\newcommand{\cB}{{\mathcal{B}}}
\newcommand{\cC}{{\mathcal{C}}}
\newcommand{\cD}{{\mathcal{D}}}
\newcommand{\cE}{{\mathcal{E}}}
\newcommand{\cF}{{\mathcal{F}}}
\newcommand{\cH}{{\mathcal{H}}}
\newcommand{\cM}{{\mathcal{M}}}
\newcommand{\cN}{{\mathcal{N}}}
\newcommand{\cR}{{\mathcal{R}}}
\newcommand{\cV}{{\mathcal{V}}}
\newcommand{\cCM}{{\mathcal{C}'}}

\newcommand{\bsa}{{\boldsymbol{a}}}
\newcommand{\bsb}{{\boldsymbol{b}}}
\newcommand{\bsc}{{\boldsymbol{c}}}
\newcommand{\bsg}{{\boldsymbol{g}}}
\newcommand{\bsm}{{\boldsymbol{m}}}
\newcommand{\bsu}{{\boldsymbol{u}}}
\newcommand{\bsv}{{\boldsymbol{v}}}
\newcommand{\bsw}{{\boldsymbol{w}}}
\newcommand{\bsx}{{\boldsymbol{x}}}
\newcommand{\bsy}{{\boldsymbol{y}}}
\newcommand{\bsz}{{\boldsymbol{z}}}

\newcommand{\bsepsilon}{{\boldsymbol{\epsilon}}}
\newcommand{\bszero}{{\boldsymbol{0}}}
\newcommand{\bsalpha}{{\boldsymbol{\alpha}}}
\newcommand{\bsbeta}{{\boldsymbol{\beta}}}
\newcommand{\bspsi}{{\boldsymbol{\psi}}}
\newcommand{\bsphi}{{\boldsymbol{\phi}}}
\newcommand{\bsvarphi}{{\boldsymbol{\varphi}}}
\newcommand{\bseta}{{\boldsymbol{\eta}}}
\newcommand{\bstheta}{{\boldsymbol{\theta}}}

\newcommand{\red}[1]{{\color{red}{#1}}}
\newcommand{\green}[1]{{\color{green}{#1}}}

\newtheorem{theorem}{Theorem}
\newtheorem{assumption}{Assumption}
\newtheorem{remark}{Remark}


==> numerics.tex <==

\section{Numerical experiment}
% We consider the Tumor growing model. The accuracy of the predictions $\dy_i$ and $\frac{\partial \dy_i}{\partial\dm}$ for $i = 1, \dots, N$ is problem-dependent. We will demonstrate the accuracy of the neural network for each example.

\subsection{Tumor equation}
The tumor model is developed to understand tumor proliferation and infiltration. Specifically, we focus on Glioblastoma, the most aggressive primary brain tumor. Medical imaging techniques often struggle to identify the boundary of the tumor precisely, potentially leading to suboptimal interventions and prognoses \cite{stupp2005radiotherapy, liang2023image}.

In clinical practice, obtaining daily MRI images (e.g., ten days) would provide the most comprehensive information for treatment planning. However, this approach is time-consuming and expensive. Identifying the most informative time points for MRI imaging can be approached as a sequential experimental design problem. To evaluate the effectiveness of our proposed method, we utilize the example presented in \cite{liang2023image}.

For the tumor growth model, we use a reaction-diffusion partial differential equation:

\begin{align}
    \frac{\partial u}{\partial t} = \nabla \cdot (D \nabla u) + G (1 - u) u& \ \ \ \ \text{ in } \Omega \times (0, T],\\
    D \nabla u \cdot n = 0& \ \ \ \ \text{ on } \partial \Omega \times (0, T],\\
    u(x,0) = u_0& \ \ \ \ \text{ in } \Omega,
\end{align}
where $\Omega$ denotes the brain domain of a specific rat extracted from a segmented 2D slice of a T2-weighted MRI image, the function $u(x,t) \in [0,1]$ quantifies the estimated tumor volume fraction at position $x$ and time $t$. The parameter $D(x)$ characterizes tumor diffusion, encompassing invasion and cell migration processes, while $G(x)$ represents the tumor's growth rate, capturing the proliferation of tumor cells through division and expansion.

We adopt the parameters from \cite{liang2023image} to define the prior distribution. The brain is divided into gray and white matter, each with distinct characteristics. Table \ref{table:params} define the different mean, different $\gamma$, and $\delta$ values in the Mat\'ern covariance operator for these two regions: 

\begin{equation}   
\delta = \frac{\sqrt{2}}{\sigma \rho \sqrt{\pi}}, \ \gamma = \frac{1}{4\sqrt{2\pi}}\frac{\rho}{\sigma}.
\end{equation}

\begin{table}
\centering
\caption{Estimated hyper-parameters for the tumor model}
\begin{tabular}{cc|cc}
\hline
\multicolumn{4}{c}{Prior mean and variance of parameters} \\
\hline
\multicolumn{2}{c|}{$\log(G_\text{gm})$} & \multicolumn{2}{c}{$\log(G_\text{wm})$} \\
\multicolumn{2}{c|}{$\log(1/\text{day})$} & \multicolumn{2}{c}{$\log(1/\text{day})$} \\
Mean & Variance & Mean & Variance \\
\hline
-0.7800 & 0.0682 & -0.8419 & 0.0682 \\
\hline
\multicolumn{4}{c}{Spatial correlation lengths of $\dm$} \\
\hline
\multicolumn{2}{c|}{$\rho_\text{gm}$ (mm)} & \multicolumn{2}{c}{$\rho_\text{wm}$ (mm)} \\
\multicolumn{2}{c|}{6.0} & \multicolumn{2}{c}{12.0} \\
\hline
\end{tabular} \label{table:params}
\end{table}

In this problem, we use $G(x)$ as a Gaussian random field, while $D(x)$ is treated as a constant with $\log(D_\text{gm}) = -0.9937, \log(D_\text{wm}) = -0.3006$. While the proposed neural network can be tuned to fit two model parameters, we initially focus on the reaction term coefficient as the primary model parameter. Using these parameters, we generate the prior samples in the rat's brain domain, as illustrated in Figure \ref{fig:3plots}
\begin{figure}
    \centering
    \includegraphics[width=0.3\textwidth]{Figures/brain.png}
    \hspace{0.02\textwidth}
    \includegraphics[width=0.3\textwidth]{Figures/prior_mean.png}
    \hspace{0.02\textwidth}    
    \includegraphics[width=0.30\textwidth]{Figures/G_plot.png}
   \caption{Left: Illustration of gray and white matter in a rat's brain. Middle: Prior mean $\dm_\text{prior}$. Right: A random prior sample $\dm \sim \mathcal{N} (\dm_\text{prior}, \Gamma_\text{prior})$.}
    \label{fig:3plots}
\end{figure}

\subsubsection{Observation}

We use the initial condition, which represents the implantation of the tumor in the brain, as a starting point. We then solve the PDE problems and visualize the solutions. Figure \ref{fig:states} illustrates the tumor growth and spread as governed by the equation.

\begin{figure}
    \centering
    \includegraphics[width=0.3\textwidth]{Figures/init.png}
    \hspace{0.02\textwidth}
    \includegraphics[width=0.3\textwidth]{Figures/2_step.png}
    \hspace{0.02\textwidth}    
    \includegraphics[width=0.30\textwidth]{Figures/5_step.png}
   \caption{Left: Initial tumor state. Middle: Tumor state at step 2. Right: Tumor state at step 5.}
    \label{fig:states}
\end{figure}

\subsection{Dimension reduction}

The model parameter dimension and tumor solution are in a high-dimensional space of 14,003 dimensions. Training all the model parameters and the entire output space would be inefficient. Therefore, we first examine the eigenvalues and singular values of the DIS and PCA. Figure \ref{fig:eigenvalues} shows that the eigenvalues decrease rapidly, indicating that we can effectively use just 128 components for both the model parameters and outputs. Figure \ref{fig:modes} illustrates the eigenvectors of each subspace.

\begin{figure}
    \centering
        \includegraphics[width=0.3\textwidth]{Figures/pca-eigval.png} 
        \includegraphics[width=0.3\textwidth]{Figures/dis-eigvals.png} 
    \caption{Left: PCA singular values, Right: DIS eigenvalues}
    \label{fig:eigenvalues}
\end{figure}


\begin{figure}
    \centering
    \begin{tabular}{ccc}
        \includegraphics[width=0.3\textwidth]{Figures/pca-1.png} &
        \includegraphics[width=0.3\textwidth]{Figures/pca-2.png} &
        \includegraphics[width=0.3\textwidth]{Figures/pca-4.png} \\
        \includegraphics[width=0.3\textwidth]{Figures/dis-1.png} &
        \includegraphics[width=0.3\textwidth]{Figures/dis-2.png} &
        \includegraphics[width=0.3\textwidth]{Figures/dis-4.png}
    \end{tabular}
    \caption{PCA modes (Top) and DIS modes (Bottom)}
    \label{fig:modes}
\end{figure}

\subsection{The proposed neural network performance}
After reducing the dimensions of the model parameters and output space, we train the neural network $F_{NN, i}$ as described in Section \ref{sec:nn}. With the 1024 training samples, we train the proposed neural network. For evaluating the neural network performance, we use the relative error:
\begin{equation}\label{eq:errorFJ}
  \mathbb{E}_{\dm} \left[ \frac{\|F_i(\dm) - F_{NN,i}(\dm)\|_{M}}{\|F_i(\dm)\|_{M}}\right] \text{ and } \mathbb{E}_{\dm} \left[ \frac{\|J_i(\dm) - J_{NN,i}(\dm)\|_F}{\|J_i(\dm)\|_F}\right],
\end{equation}
where $M$ denotes the mass matrix, and $\|\cdot\|_F$ represents the Frobenius norm.

\begin{figure}
    \centering
    \begin{tabular}{cccc}
        \includegraphics[width=0.24\textwidth]{Figures/nn_1.png} &
        \includegraphics[width=0.24\textwidth]{Figures/nn_2.png} &
        \includegraphics[width=0.24\textwidth]{Figures/nn_4.png} &
        \includegraphics[width=0.24\textwidth]{Figures/nn_8.png} \\
        \includegraphics[width=0.24\textwidth]{Figures/fem_1.png} &
        \includegraphics[width=0.24\textwidth]{Figures/fem_2.png} &
        \includegraphics[width=0.24\textwidth]{Figures/fem_4.png} &
        \includegraphics[width=0.24\textwidth]{Figures/fem_8.png} \\
        \includegraphics[width=0.24\textwidth]{Figures/nn_fem_1.png} &
        \includegraphics[width=0.24\textwidth]{Figures/nn_fem_2.png} &
        \includegraphics[width=0.24\textwidth]{Figures/nn_fem_4.png} &
        \includegraphics[width=0.24\textwidth]{Figures/nn_fem_8.png} \\
    \end{tabular}
    \caption{Comparison of NN and FEM outputs: NN output (Top), FEM output (Middle), and NN - FEM difference (Bottom) for steps 1, 2, 4, and 8}
    \label{fig:nn_fem_comparison}
\end{figure}

\subsubsection{MAP point comparison}
\begin{equation}
  \E_{\dy} \left[ \frac{||\dm_{\text{MAP}}^{\dy, \xi} - P_r(\dm_{\text{MAP}}^{\dy, \xi})||_M}{||\dm_{\text{MAP}}^{\dy, \xi}||_M}\right]\label{eq:MAP-re}
\end{equation}

We compute the MAP point using the full observations
\begin{figure}
    \centering
        \includegraphics[width=0.3\textwidth]{Figures/FEM_MAP.png} 
        \includegraphics[width=0.3\textwidth]{Figures/NN_MAP.png} 
        \includegraphics[width=0.3\textwidth]{Figures/NN_FEM_MAP.png} 
    \caption{Left: FEM MAP point, Middle: NN MAP point, Right: Difference}
    \label{fig:MAP-compare}
\end{figure}

We also compute the MAP using [2,5,8] times
\begin{figure}
    \centering
        \includegraphics[width=0.3\textwidth]{Figures/FEM_MAP_258.png} 
        \includegraphics[width=0.3\textwidth]{Figures/NN_MAP_258.png} 
        \includegraphics[width=0.3\textwidth]{Figures/NN_FEM_MAP_258.png} 
    \caption{Left: FEM MAP point, Middle: NN MAP point, Right: Difference}
    \label{fig:MAP-compare}
\end{figure}
\subsubsection{The proposed method result}
-Greedy
-Total EIG
uncertainty decrease



\subsubsection{Uncertainty decreases}
\begin{figure}
    \centering
        \includegraphics[width=0.3\textwidth]{Figures/unc-prior.png} 
        \includegraphics[width=0.3\textwidth]{Figures/unc-dec-opt.png} 
        \includegraphics[width=0.3\textwidth]{Figures/unc-dec-uni.png} 
    \caption{Left: Prior, Middle: Optimal, Right: Uniform}
    \label{fig:MAP-compare}
\end{figure}

\subsection{Diffusion equation or Convection-Diffusion-Reaction equation}

